Generative Adversarial Networks (GANs): What it can generate and What it cannot?

In recent years, Generative Adversarial Networks (GANs) have received significant attention from the research community. With a straightforward implementation and outstanding results, GANs have been used for numerous applications. Despite the success, GANs lack a proper theoretical explanation. These models suffer from issues like mode collapse, non-convergence, and instability during training. To address these issues, researchers have proposed theoretically rigorous frameworks inspired by varied fields of Game theory, Statistical theory, Dynamical systems, etc. In this paper, we propose to give an appropriate structure to study these contributions systematically. We essentially categorize the papers based on the issues they raise and the kind of novelty they introduce to address them. Besides, we provide insight into how each of the discussed articles solves the concerned problems. We compare and contrast different results and put forth a summary of theoretical contributions about GANs with focus on image/visual applications. We expect this summary paper to give a bird's eye view to a person wishing to understand the theoretical progress in GANs so far.

==> table.tex <==
\centering
% \Rotatebox{90}{%
\captionof{table}{\textbf{Summary of GAN Papers}}
\begin{adjustbox}{max width = 9cm}
\label{tab:2}
\begin{tabular}{|l|l|l|l|}
\hline 
 \textbf{Paper Name }& \textbf{Problems Raised} & \textbf{Novel approach} & \textbf{Comment} \\\hline
On Distinguish-ability Criteria & \textcolor{purple}{ The expected gradient of generator}  & \textcolor{purple}{In gans G being the primary model} &  \\
   For Estimating& \textcolor{purple}{does not  match that of MLE.}&\textcolor{purple}{causes it to differ from MLE.}& \\
Generative Models \cite{2014Goodfellow} & Non convergence of independent SGD& No close relation between NCE and GAN.& \\
&results in under-fitting in gans& &\\
&&& \\
June & Improved Techniques  & \textcolor{red}{Overtraining of the discriminator}  & \textcolor{red}{Feature Matching}  \\
2016 &for GANs \cite{goodfellow16} &\textcolor{purple}{Mode collapse of Generator} & \textcolor{purple}{Mini-batch Discrimination} \\
&& \textcolor{orange}{Gradient descent may not converge} & \textcolor{orange}{Historical Averaging (Fictitious play)}\\
& & \textcolor{magenta}{Vulnerable to adversarial examples.} & \textcolor{magenta}{Label-smoothing} \\
&&\textcolor{brown}{GAN outputs depend on the inputs} & \textcolor{brown}{Virtual Batch normalization} \\
&& \textcolor{brown}{within a same batch due to BN} &\\
& & & \\
Jan& Towards Principled Methods & \textcolor{purple}{Perfect Discriminator resulting in} & \textcolor{purple}{Softer Metrics- Adding Gaussian}\\
2017 &for Training GANs \cite{arjovsky01} & \textcolor{purple}{zero grads when distributions are  in} & \textcolor{purple}{Noise (Contrastive Divergence)} \\
&&\textcolor{purple}{dimensional manifolds}& \textcolor{purple}{Earth-Mover Distance}\\
&&The $-\log D$ alternative causes-  & \\
&&unstable updates& \\
& & & \\
Mar & WGAN \cite{arjovskyWGAN}& Learning distributions supported& Define EM Distance (KR Duality) with well  \\
2017 && in lower dimension manifolds.& defined gradients and avoids balancing \\
&& JSD maxes and $KL\rightarrow\infty$& the critic and generator. Consistent decrease\\
&& Mode Collapse &in loss with training. Weakest metric\\
&&& \\
May & Improved Techniques &Lipschitz enforced by weight clipping. & Introduced a Gradient Penalty term. \\
2017 &on WGAN  \cite{gularajani} & Capacity underuse (critic has high & wrt sample as following was observed.\\
& & bias), Exploding and&Optimal critic has unit-grad \\
&& vanishing gradients. & norm between $\mathbb{P}_{r}$ and $\mathbb{P}_{g}$\\
& & & \\

Mar& Loss-Sensitive GAN on & \textcolor{purple}{Over-pessimistic D as fake samples} & \textcolor{purple}{Loss having a data-dependent margin.} \\
2017& Lipschitz Densities\cite{ls-gan}& \textcolor{purple}{closer to data are still negative} & \\
&&\textcolor{magenta}{Assuming infinite capacity which leads}& \textcolor{magenta}{Limited to the space of}\\
&&\textcolor{magenta}{to mode collapse and vanishing grads}&\textcolor{magenta}{Lipschitz-continuous functions}\\
&&\textcolor{orange}{WGAN is unbounded from above as} & \textcolor{orange}{Pairwise comparisons as against WGAN}\\
&& \textcolor{orange}{critic is minimized over gen samples}&\textcolor{orange}{which decomposes the loss}\\
&&&\textcolor{orange}{into two first order moments}\\
&&&\\
& & & \\
ICLR & EBGAN \cite{eb-gan} & With binary logistic loss only two & Auto-encoder Discriminator to evade    \\
2017 & &targets are possible, so gradients in & the need of negative samples \\
&&a mini batch are far from orthogonal.& Repelling regularizer \\
&&Mode Collapse.& to prevent mode collapse\\
& & & \\

Feb & Least Squares GAN \cite{lsgan}& Vanishing gradients with sigmoid & Pearson $\chi^2$ Divergence. The following  \\
2017&&cross-entropy loss when updating & constants , a- encoding for real data\\
&&the gen using fake samples&b - encoding for fake data \\
&&that are on the correct side & c- encoding for value that G wants\\
&&of decision boundary.& D to believe is fake.\\
&&&\\
June & f-GAN\cite{fgan}&   & General $f$-divergence \\
2016&&\textcolor{red}{No convergence to saddle point} & variational estimation of $f-$ divergence \\
&&\textcolor{red}{when using single step GD} & \textcolor{red}{Variational Divergence Minimization}\\
&&& \\
Nov & Stabilizing Training of\cite{fgan_2} & Empirical estimation& Convolving with noise \\
2017 &  GANs through Regularization & Density misspecification& Noise induced regularization \\
&&Dimensional misspecification &\\
&&Addition of high dim noise introduces &\\
&&huge variance in parameter estimation&\\
&&&\\
NIPS& The Numerics of GANs \cite{geiger06} & Failure of simultaneous  &
Consensus Optimization: Alternative method  \\
 2017 & &gradient descent as the eigenvalues &  for finding the Nash Equilibrium\\
 &&gradients have zero real part &Introduced norm of the gradients\\
 &&and large imaginary part&w.r.t parameters in the loss.\\
 
% \hline 
% \end{tabular}
% \end{adjustbox}
% \newpage

% \begin{adjustbox}{max width = 9cm}
% \begin{tabular}{|l|l|l|l|}
% \hline
Nov&Unrolled GANs \cite{unrolled} & Mode collapse, Oscillations& Training the D to optimality\\
2016&&of G and D. G tries to move much mass to single & is expensive.A surrogative loss \\
&&point, D tracks it and assigns lower probability& which in limit equals optimal D \\
&&The cycle continues forever.& The G's updates consider future\\
&&&steps of the discriminator.\\
&&&\\
Aug& Generalization and Equilibrium &\textcolor{purple}{Generalization is not guaranteed i.e.} &\textcolor{purple}{NN Distance which generalizes} \\
2017 &in GANs \cite{Arora03}&\textcolor{purple}{$d(\mathcal{D}_{real}, \mathcal{D}) = 0$ but  $d(\mathcal{\hat{D}}_{real}, \mathcal{\hat{D}}) \neq 0$}&\textcolor{purple}{as it assumes finite capacity D} \\
&& \textcolor{purple}{where $\hat{D}$ is the empirical distribution} & \textcolor{purple}{At the cost of diversity of samples.}\\
&&\textcolor{red}{Non Existence of equilibrium in GAN} &\textcolor{red}{Mixed Strategy Nash using}  \\
&&&\textcolor{red}{mixture of Generators which} \\
&&& \textcolor{red}{on folding results in pure NE.}\\
&&&\\
May & On Convergence and Stability& Gradient descent is unstable and & Regret Minimization converges to  \\
 2017 & in GANs \cite{DRAGAN} &results in mode collapse &$\epsilon$-equilibrium in non-convex case.  \\
& &Divergence minimization hypothesis doesn't  & Sharp gradients results in  \\ 
&& explain gan learning swiss roll distribution & mode collapse hence a penalty\\
&&WGAN and LS-GAN regularize the discriminator's& term is introduced.\\
&&gradients in domain space.&\\
&&&\\
Nov & Gradient Descent GAN & It is assumed that updates occur  & local asymptotic stability of GAN  \\
 2017 &  Optimization is locally stable & in functional space, with models having & 
(not WGAN)  optimization under   \\
&  &infinite capacity. Discriminator is assumed  & 
proper conditions, gradient-based  \\
&  &to be fully optimized between gen updates.  & 
 regularizer(GAN + WGAN)  \\
&&&\\
\hline 
\end{tabular}
\end{adjustbox}
